Get me out of this hole: Identifying and avoiding inferior local optima in choice models

Choice modellers routinely acknowledge the risk of convergence to inferior local optima when using structures other than a simple linear-in-parameters logit model, but there is no consensus on how to address it. Most analysts seem to ignore the problem, while others try a set of different starting values or put their faith in what they believe to be more robust estimation approaches. This paper puts the question on a firmer empirical footing for latent class models, contrasting eight estimation strategies on a stated choice and a revealed preference dataset. These include multistart, global optimisation heuristics, the EM algorithm, and a proposed new profile likelihood algorithm that systematically analyses the parameter space around an initial estimate in search of better optima. Multiple well identified local optima are present in both case studies, with eight distinct solutions in the first and $23$ in the second, and no single approach recovers all of them. The solution that is easiest to find is not the one that fits best, and conventional starting values lead to a solution ranking thirteenth of $23$ in the second case study. We further show why these optima exist, tracing the barriers in log-likelihood between solutions to an interchange of substantive roles between classes. The consequences are material: willingness-to-pay measures differ by up to $60\%$ across solutions and elasticities by a factor of two, with the ordering of solutions by fit bearing little relation to their ordering by any such measure.

==> source/2_DECISIONS/outputs_5_estimation_results_table.tex <==
\begin{table}[!h]
\centering
\caption{Estimation results on DECISIONS mode choice data for selected solutions, sorted in increasing order of LL. Best-fitting solution: Best ($S^{(3)}$) with LL = -2,869.66.}
\label{tab:decisions_results}
\centering
\adjustbox{max width=\linewidth,max totalheight=\textheight}{
\fontsize{8}{10}\selectfont
\begin{tabular}[t]{llrrrrrr}
\toprule
\multicolumn{2}{c}{ } & \multicolumn{2}{c}{Base ($S^{(1)}$)} & \multicolumn{2}{c}{Most frequent ($S^{(4)}$)} & \multicolumn{2}{c}{Best ($S^{(3)}$)} \\
\cmidrule(l{3pt}r{3pt}){3-4} \cmidrule(l{3pt}r{3pt}){5-6} \cmidrule(l{3pt}r{3pt}){7-8}
 &  & Estimate & Rob. t-ratio & Estimate & Rob. t-ratio & Estimate & Rob. t-ratio\\
\midrule
\multicolumn{2}{l}{LL(final)} & \multicolumn{2}{c}{-2,906.05} & \multicolumn{2}{c}{-2,869.84} & \multicolumn{2}{c}{-2,869.66} \\
\multicolumn{2}{l}{BIC} & \multicolumn{2}{c}{6,070.98} & \multicolumn{2}{c}{5,998.56} & \multicolumn{2}{c}{5,998.20} \\
\midrule
 & $\alpha_{car,1}$ & 0.0000 & N/A & 0.0000 & N/A & 0.0000 & N/A\\

\multirow[t]{-2}{*}{\raggedright\arraybackslash ASC (car)} & $\alpha_{car,2}$ & 0.0000 & N/A & 0.0000 & N/A & 0.0000 & N/A\\

 & $\alpha_{bus,1}$ & -1.1865 & -2.74 & -4.6530 & -6.82 & -5.0530 & -6.60\\

\multirow[t]{-2}{*}{\raggedright\arraybackslash ASC (bus)} & $\alpha_{bus,2}$ & -3.9517 & -5.15 & -1.7508 & -4.61 & -1.2391 & -3.69\\

 & $\alpha_{rail,1}$ & -1.4832 & -1.18 & -2.5237 & -4.32 & -2.8087 & -4.49\\

\multirow[t]{-2}{*}{\raggedright\arraybackslash ASC (rail)} & $\alpha_{rail,2}$ & -2.4765 & -4.64 & -1.7170 & -2.79 & -1.4556 & -2.08\\

 & $\alpha_{taxi,1}$ & -1.5173 & -1.17 & -2.7107 & -6.19 & -3.3105 & -7.90\\

\multirow[t]{-2}{*}{\raggedright\arraybackslash ASC (taxi)} & $\alpha_{taxi,2}$ & -4.3232 & -7.89 & -4.5895 & -6.86 & -3.9113 & -5.98\\

 & $\alpha_{cycling,1}$ & -3.5640 & -4.85 & -3.7396 & -7.13 & -4.2386 & -8.32\\

\multirow[t]{-2}{*}{\raggedright\arraybackslash ASC (cycling)} & $\alpha_{cycling,2}$ & -4.0506 & -3.84 & -5.9804 & -6.83 & -5.4237 & -6.44\\

 & $\alpha_{walking,1}$ & 0.1794 & 0.34 & -0.1538 & -0.43 & 0.0736 & 0.17\\

\multirow[t]{-2}{*}{\raggedright\arraybackslash ASC (walking)} & $\alpha_{walking,2}$ & 0.0169 & 0.05 & 0.0720 & 0.16 & 0.2292 & 0.57\\

 & $\beta_{tt\,car,1}$ & -0.1621 & -5.68 & -0.1298 & -5.87 & -0.1347 & -6.12\\

\multirow[t]{-2}{*}{\raggedright\arraybackslash In-vehicle time (car)} & $\beta_{tt\,car,2}$ & -0.1357 & -9.01 & -0.1820 & -6.40 & -0.1796 & -5.47\\

 & $\beta_{tt\,bus,1}$ & -0.0448 & -2.86 & -0.0354 & -2.69 & -0.0302 & -2.49\\

\multirow[t]{-2}{*}{\raggedright\arraybackslash In-vehicle time (bus)} & $\beta_{tt\,bus,2}$ & -0.0344 & -3.10 & -0.0521 & -4.71 & -0.0591 & -4.81\\

 & $\beta_{tt\,rail,1}$ & -0.0410 & -1.31 & -0.0147 & -0.65 & -0.0160 & -0.76\\

\multirow[t]{-2}{*}{\raggedright\arraybackslash In-vehicle time (rail)} & $\beta_{tt\,rail,2}$ & -0.0567 & -3.22 & -0.0837 & -4.17 & -0.0888 & -4.10\\

 & $\beta_{tt\,taxi,1}$ & -0.1402 & -2.04 & -0.1830 & -4.27 & -0.1709 & -3.98\\

\multirow[t]{-2}{*}{\raggedright\arraybackslash In-vehicle time (taxi)} & $\beta_{tt\,taxi,2}$ & -0.1366 & -2.97 & -0.0541 & -1.32 & -0.0627 & -1.41\\

 & $\beta_{tt\,cycling,1}$ & -0.0679 & -4.36 & -0.0741 & -5.01 & -0.0690 & -4.67\\

\multirow[t]{-2}{*}{\raggedright\arraybackslash Travel time (cycling)} & $\beta_{tt\,cycling,2}$ & -0.3146 & -2.57 & -0.1324 & -2.57 & -0.1391 & -2.48\\

 & $\beta_{tt\,walking,1}$ & -0.1724 & -6.24 & -0.1162 & -6.08 & -0.1632 & -6.76\\

\multirow[t]{-2}{*}{\raggedright\arraybackslash Travel time (walking)} & $\beta_{tt\,walking,2}$ & -0.1348 & -8.80 & -0.1614 & -8.01 & -0.1232 & -6.84\\

 & $\beta_{ovt\,bus,1}$ & -0.1747 & -4.27 & -0.1349 & -3.34 & -0.1381 & -3.23\\

\multirow[t]{-2}{*}{\raggedright\arraybackslash Out-of-vehicle time (bus)} & $\beta_{ovt\,bus,2}$ & -0.1243 & -4.73 & -0.1430 & -8.69 & -0.1368 & -8.82\\

 & $\beta_{ovt\,rail,1}$ & -0.1275 & -2.72 & -0.0906 & -4.96 & -0.0900 & -5.00\\

\multirow[t]{-2}{*}{\raggedright\arraybackslash Out-of-vehicle time (rail)} & $\beta_{ovt\,rail,2}$ & -0.0991 & -6.81 & -0.1283 & -4.10 & -0.1274 & -3.49\\

 & $\beta_{tc,1}$ & -0.6001 & -2.95 & -0.2010 & -4.62 & -0.1953 & -4.15\\

\multirow[t]{-2}{*}{\raggedright\arraybackslash Cost} & $\beta_{tc,2}$ & -0.0402 & -1.03 & -0.2295 & -3.36 & -0.2406 & -3.24\\

 & $\delta_1$ & 0.0000 & N/A & 0.0000 & N/A & 0.0000 & N/A\\

\multirow[t]{-2}{*}{\raggedright\arraybackslash Class allocation delta} & $\delta_2$ & 0.6570 & 2.41 & -0.4684 & -1.64 & -0.5133 & -2.11\\

\cdashline{1-8}
 & Class 1 & 0.3414 & 5.57 & 0.6150 & 9.08 & 0.6256 & 10.99\\

\multirow[t]{-2}{*}{\raggedright\arraybackslash Class allocation weight} & Class 2 & 0.6586 & 10.74 & 0.3850 & 5.69 & 0.3744 & 6.58\\

\cdashline{1-8}
 & Class 1 & 16.2087 & 2.48 & 38.7395 & 3.52 & 41.3755 & 3.42\\

 & Class 2 & 202.2941 & 1.01 & 47.5937 & 3.02 & 44.7842 & 3.20\\

 & Weighted average & 138.7619 & 1.09 & 42.1483 & 5.21 & 42.6518 & 5.12\\

 & Difference in mean & \multicolumn{2}{c}{+225.34\%} & \multicolumn{2}{c}{-1.18\%} & \multicolumn{2}{c}{N/A} \\

 & Std. dev. in sample & 88.2387 & 0.92 & 4.3084 & 0.43 & 1.6497 & 0.17\\

\multirow[t]{-6}{*}{\raggedright\arraybackslash Value of in-vehicle time, car (\pounds/hour)} & Difference in std. dev. & \multicolumn{2}{c}{+5248.77\%} & \multicolumn{2}{c}{+161.16\%} & \multicolumn{2}{c}{N/A} \\

 & Class 1 & 4.4841 & 1.65 & 10.5651 & 2.30 & 9.2693 & 2.10\\

 & Class 2 & 51.3606 & 1.08 & 13.6295 & 3.22 & 14.7402 & 3.41\\

 & Weighted average & 35.3563 & 1.15 & 11.7449 & 3.75 & 11.3176 & 3.80\\

 & Difference in mean & \multicolumn{2}{c}{+212.40\%} & \multicolumn{2}{c}{+3.78\%} & \multicolumn{2}{c}{N/A} \\

 & Std. dev. in sample & 22.2281 & 0.98 & 1.4911 & 0.48 & 2.6478 & 0.84\\

\multirow[t]{-6}{*}{\raggedright\arraybackslash Value of in-vehicle time, bus (\pounds/hour)} & Difference in std. dev. & \multicolumn{2}{c}{+739.49\%} & \multicolumn{2}{c}{-43.69\%} & \multicolumn{2}{c}{N/A} \\

 & Class 1 & 4.0965 & 1.11 & 4.3926 & 0.61 & 4.9099 & 0.70\\

 & Class 2 & 84.4974 & 0.90 & 21.8797 & 2.72 & 22.1300 & 2.69\\

 & Weighted average & 57.0474 & 0.95 & 11.1250 & 2.23 & 11.3573 & 2.26\\

 & Difference in mean & \multicolumn{2}{c}{+402.30\%} & \multicolumn{2}{c}{-2.05\%} & \multicolumn{2}{c}{N/A} \\

 & Std. dev. in sample & 38.1248 & 0.85 & 8.5091 & 1.60 & 8.3340 & 1.49\\

\multirow[t]{-6}{*}{\raggedright\arraybackslash Value of in-vehicle time, rail (\pounds/hour)} & Difference in std. dev. & \multicolumn{2}{c}{+357.46\%} & \multicolumn{2}{c}{+2.10\%} & \multicolumn{2}{c}{N/A} \\

 & Class 1 & 14.0184 & 1.56 & 54.6126 & 2.76 & 52.5142 & 2.52\\

 & Class 2 & 203.6795 & 0.85 & 14.1517 & 1.17 & 15.6304 & 1.21\\

 & Weighted average & 138.9265 & 0.91 & 39.0353 & 3.08 & 38.7044 & 2.89\\

 & Difference in mean & \multicolumn{2}{c}{+258.94\%} & \multicolumn{2}{c}{+0.85\%} & \multicolumn{2}{c}{N/A} \\

 & Std. dev. in sample & 89.9343 & 0.79 & 19.6880 & 1.63 & 17.8507 & 1.39\\

\multirow[t]{-6}{*}{\raggedright\arraybackslash Value of in-vehicle time, taxi (\pounds/hour)} & Difference in std. dev. & \multicolumn{2}{c}{+403.81\%} & \multicolumn{2}{c}{+10.29\%} & \multicolumn{2}{c}{N/A} \\

 & Class 1 & 17.4723 & 5.64 & 40.2602 & 3.11 & 42.4384 & 2.49\\

 & Class 2 & 185.3316 & 0.97 & 37.3767 & 3.35 & 34.1184 & 3.22\\

 & Weighted average & 128.0220 & 1.06 & 39.1501 & 4.12 & 39.3233 & 3.66\\

 & Difference in mean & \multicolumn{2}{c}{+225.56\%} & \multicolumn{2}{c}{-0.44\%} & \multicolumn{2}{c}{N/A} \\

 & Std. dev. in sample & 79.5962 & 0.87 & 1.4031 & 0.18 & 4.0266 & 0.38\\

\multirow[t]{-6}{*}{\raggedright\arraybackslash Value of out-of-vehicle time, bus (\pounds/hour)} & Difference in std. dev. & \multicolumn{2}{c}{+1876.76\%} & \multicolumn{2}{c}{-65.15\%} & \multicolumn{2}{c}{N/A} \\

 & Class 1 & 12.7515 & 2.50 & 27.0463 & 3.64 & 27.6606 & 3.48\\

 & Class 2 & 147.7129 & 0.98 & 33.5556 & 2.62 & 31.7558 & 2.59\\

 & Weighted average & 101.6351 & 1.06 & 29.5524 & 4.80 & 29.1939 & 4.65\\

 & Difference in mean & \multicolumn{2}{c}{+248.14\%} & \multicolumn{2}{c}{+1.23\%} & \multicolumn{2}{c}{N/A} \\

 & Std. dev. in sample & 63.9965 & 0.89 & 3.1674 & 0.42 & 1.9820 & 0.27\\

\multirow[t]{-6}{*}{\raggedright\arraybackslash Value of out-of-vehicle time, rail (\pounds/hour)} & Difference in std. dev. & \multicolumn{2}{c}{+3128.88\%} & \multicolumn{2}{c}{+59.81\%} & \multicolumn{2}{c}{N/A} \\

 & Class 1 & 6.7841 & 2.96 & 22.1292 & 3.42 & 21.2021 & 3.24\\

 & Class 2 & 468.9996 & 0.97 & 34.6054 & 2.13 & 34.6845 & 2.12\\

 & Weighted average & 311.1926 & 1.01 & 26.9325 & 3.88 & 26.2501 & 3.76\\

 & Difference in mean & \multicolumn{2}{c}{+1085.49\%} & \multicolumn{2}{c}{+2.60\%} & \multicolumn{2}{c}{N/A} \\

 & Std. dev. in sample & 219.1752 & 0.94 & 6.0709 & 0.69 & 6.5251 & 0.73\\

\multirow[t]{-6}{*}{\raggedright\arraybackslash Value of travel time, cycling (\pounds/hour)} & Difference in std. dev. & \multicolumn{2}{c}{+3258.96\%} & \multicolumn{2}{c}{-6.96\%} & \multicolumn{2}{c}{N/A} \\

 & Class 1 & 17.2384 & 3.67 & 34.6736 & 3.81 & 50.1412 & 3.33\\

 & Class 2 & 200.9440 & 1.03 & 42.1971 & 3.18 & 30.7088 & 2.97\\

 & Weighted average & 138.2242 & 1.11 & 37.5701 & 5.41 & 42.8654 & 4.95\\

 & Difference in mean & \multicolumn{2}{c}{+222.46\%} & \multicolumn{2}{c}{-12.35\%} & \multicolumn{2}{c}{N/A} \\

 & Std. dev. in sample & 87.1103 & 0.93 & 3.6609 & 0.45 & 9.4047 & 0.89\\

\multirow[t]{-6}{*}{\raggedright\arraybackslash Value of travel time, walking (\pounds/hour)} & Difference in std. dev. & \multicolumn{2}{c}{+826.24\%} & \multicolumn{2}{c}{-61.07\%} & \multicolumn{2}{c}{N/A} \\
\bottomrule
\end{tabular}}
\end{table}

